Martingale Posterior Neural Processes

A Neural Process (NP) estimates a stochastic process implicitly defined with neural networks given a stream of data, rather than pre-specifying priors already known, such as Gaussian processes. An ideal NP would learn everything from data without any inductive biases, but in practice, we often restrict the class of stochastic processes for the ease of estimation. One such restriction is the use of a finite-dimensional latent variable accounting for the uncertainty in the functions drawn from NPs. Some recent works show that this can be improved with more "data-driven" source of uncertainty such as bootstrapping. In this work, we take a different approach based on the martingale posterior, a recently developed alternative to Bayesian inference. For the martingale posterior, instead of specifying prior-likelihood pairs, a predictive distribution for future data is specified. Under specific conditions on the predictive distribution, it can be shown that the uncertainty in the generated future data actually corresponds to the uncertainty of the implicitly defined Bayesian posteriors. Based on this result, instead of assuming any form of the latent variables, we equip a NP with a predictive distribution implicitly defined with neural networks and use the corresponding martingale posteriors as the source of uncertainty. The resulting model, which we name as Martingale Posterior Neural Process (MPNP), is demonstrated to outperform baselines on various tasks.

==> table/_old_tables/table_gp_inf.tex <==
\begin{table}[t]
    \caption{Context and target log likelihood values on data sampled from Gaussian Processes with various kernel. In the last column $t$-noise data generated by adding noise sampled from student $t$ distribution to Gaussian Processes with RBF Kernel. Performances are measured over 4 seeds.\\}
    \label{tab:table_gp_inf}
    \centering
    \scriptsize
    \renewcommand{\arraystretch}{0.9}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{lrrrrrrrrrrrr}
        \toprule
        \multirow{3}{*}{Model} & \multicolumn{2}{r}{RBF}                                   & \multicolumn{2}{r}{Matern}                                & \multicolumn{2}{r}{Periodic}                                & \multicolumn{2}{r}{$t$-noise}                               \\
                                 \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                          \cmidrule(lr){6-7}                                            \cmidrule(lr){8-9}
                               & context                     & target                      & context                     & target                      & context                      & target                       & context                      & target                       \\
        \midrule
CNP                    &         0.964  $\pm{0.006}$ &         0.288  $\pm{0.006}$ &         0.859  $\pm{0.009}$ &         0.124  $\pm{0.011}$ &         -0.139  $\pm{0.007}$ &         -0.742  $\pm{0.011}$ &         -0.012  $\pm{0.021}$ &         -0.760  $\pm{0.025}$ \\
NP                     &         0.953  $\pm{0.003}$ &         0.306  $\pm{0.004}$ &         0.842  $\pm{0.015}$ &         0.133  $\pm{0.008}$ &         -0.346  $\pm{0.026}$ &         -0.698  $\pm{0.007}$ &         -0.018  $\pm{0.022}$ &         -0.656  $\pm{0.028}$ \\
BNP                    &         1.020  $\pm{0.006}$ &         0.372  $\pm{0.006}$ &         0.929  $\pm{0.008}$ &         0.206  $\pm{0.006}$ &         -0.036  $\pm{0.031}$ &         -0.738  $\pm{0.011}$ &         -0.051  $\pm{0.051}$ &         -0.670  $\pm{0.023}$ \\
NeuBNP                 &         0.929  $\pm{0.011}$ &         0.275  $\pm{0.007}$ &         0.834  $\pm{0.008}$ &         0.122  $\pm{0.004}$ &         -0.231  $\pm{0.010}$ &         -0.785  $\pm{0.023}$ &          0.038  $\pm{0.009}$ &         -0.516  $\pm{0.018}$ \\
DirectNP               &         0.876  $\pm{0.005}$ &         0.260  $\pm{0.011}$ &         0.757  $\pm{0.013}$ &         0.099  $\pm{0.015}$ &         -0.242  $\pm{0.022}$ &         -0.696  $\pm{0.004}$ &         -0.202  $\pm{0.039}$ &         -0.651  $\pm{0.013}$ \\
MPNP (ours)            & \textBF{1.086} $\pm{0.005}$ & \textBF{0.457} $\pm{0.002}$ & \textBF{1.005} $\pm{0.014}$ & \textBF{0.278} $\pm{0.006}$ & \textBF{-0.017} $\pm{0.013}$ & \textBF{-0.681} $\pm{0.009}$ & \textBF{ 0.119} $\pm{0.025}$ & \textBF{-0.381} $\pm{0.013}$ \\
\cmidrule(lr){1-1}       \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                          \cmidrule(lr){6-7}                                            \cmidrule(lr){8-9}
CANP                   &         1.372  $\pm{0.000}$ &         0.611  $\pm{0.008}$ &         1.370  $\pm{0.001}$ &         0.423  $\pm{0.004}$ &          1.168  $\pm{0.051}$ &         -0.747  $\pm{0.037}$ &          0.404  $\pm{0.057}$ &         -1.036  $\pm{0.103}$ \\
ANP                    &         1.372  $\pm{0.003}$ &         0.617  $\pm{0.027}$ &         1.372  $\pm{0.001}$ &         0.432  $\pm{0.025}$ & \textBF{ 1.178} $\pm{0.054}$ &         -0.719  $\pm{0.024}$ &          0.708  $\pm{0.054}$ &         -0.728  $\pm{0.093}$ \\
BANP                   & \textBF{1.374} $\pm{0.001}$ &         0.663  $\pm{0.002}$ &         1.371  $\pm{0.002}$ &         0.472  $\pm{0.003}$ &          0.754  $\pm{0.083}$ &         -0.913  $\pm{0.028}$ &          0.477  $\pm{0.008}$ &         -0.660  $\pm{0.059}$ \\
NeuBANP                &         1.357  $\pm{0.002}$ &         0.651  $\pm{0.005}$ &         1.352  $\pm{0.002}$ &         0.473  $\pm{0.007}$ &          0.697  $\pm{0.022}$ &         -0.779  $\pm{0.013}$ &          0.670  $\pm{0.028}$ &         -0.450  $\pm{0.014}$ \\
DirectANP              &         1.353  $\pm{0.003}$ &         0.653  $\pm{0.010}$ &         1.342  $\pm{0.009}$ &         0.430  $\pm{0.030}$ &          1.109  $\pm{0.118}$ &         -0.632  $\pm{0.031}$ &          0.254  $\pm{0.023}$ &         -0.781  $\pm{0.033}$ \\
MPANP (ours)           & \textBF{1.374} $\pm{0.000}$ & \textBF{0.698} $\pm{0.007}$ & \textBF{1.373} $\pm{0.001}$ & \textBF{0.501} $\pm{0.005}$ &          1.167  $\pm{0.047}$ & \textBF{-0.628} $\pm{0.027}$ & \textBF{ 0.773} $\pm{0.039}$ & \textBF{-0.446} $\pm{0.057}$ \\
% CNP                    &         0.964  $\pm{0.006}$ &         0.288  $\pm{0.006}$ &         0.859  $\pm{0.009}$ &         0.124  $\pm{0.011}$ &         -0.139  $\pm{0.007}$ &         -0.742  $\pm{0.011}$ &         -0.012  $\pm{0.021}$ &         -0.760  $\pm{0.025}$ \\
% NP                     &         0.953  $\pm{0.003}$ &         0.306  $\pm{0.004}$ &         0.842  $\pm{0.015}$ &         0.133  $\pm{0.008}$ &         -0.346  $\pm{0.026}$ &         -0.698  $\pm{0.007}$ &         -0.018  $\pm{0.022}$ &         -0.656  $\pm{0.028}$ \\
% BNP                    &         1.020  $\pm{0.006}$ &         0.372  $\pm{0.006}$ &         0.929  $\pm{0.008}$ &         0.206  $\pm{0.006}$ &         -0.036  $\pm{0.031}$ &         -0.738  $\pm{0.011}$ &         -0.051  $\pm{0.051}$ &         -0.670  $\pm{0.023}$ \\
% NeuBNP                 &         0.929  $\pm{0.011}$ &         0.275  $\pm{0.007}$ &         0.834  $\pm{0.008}$ &         0.122  $\pm{0.004}$ &         -0.231  $\pm{0.010}$ &         -0.785  $\pm{0.023}$ &          0.038  $\pm{0.009}$ &         -0.516  $\pm{0.018}$ \\
% MPNP (ours)            & \textBF{1.086} $\pm{0.005}$ & \textBF{0.457} $\pm{0.002}$ & \textBF{1.005} $\pm{0.014}$ & \textBF{0.278} $\pm{0.006}$ & \textBF{-0.017} $\pm{0.013}$ & \textBF{-0.681} $\pm{0.009}$ & \textBF{ 0.119} $\pm{0.025}$ & \textBF{-0.381} $\pm{0.013}$ \\
% \cmidrule(lr){1-1}       \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                          \cmidrule(lr){6-7}                                            \cmidrule(lr){8-9}
% CANP                   &         1.372  $\pm{0.000}$ &         0.611  $\pm{0.008}$ &         1.370  $\pm{0.001}$ &         0.423  $\pm{0.004}$ &          1.168  $\pm{0.051}$ &         -0.747  $\pm{0.037}$ &          0.404  $\pm{0.057}$ &         -1.036  $\pm{0.103}$ \\
% ANP                    &         1.372  $\pm{0.003}$ &         0.617  $\pm{0.027}$ &         1.372  $\pm{0.001}$ &         0.432  $\pm{0.025}$ & \textBF{1.178}  $\pm{0.054}$ &         -0.719  $\pm{0.024}$ &          0.708  $\pm{0.054}$ &         -0.728  $\pm{0.093}$ \\
% BANP                   & \textBF{1.374} $\pm{0.001}$ &         0.663  $\pm{0.002}$ &         1.371  $\pm{0.002}$ &         0.472  $\pm{0.003}$ &          0.754  $\pm{0.083}$ &         -0.913  $\pm{0.028}$ &          0.477  $\pm{0.008}$ &         -0.660  $\pm{0.059}$ \\
% NeuBANP                &         1.357  $\pm{0.002}$ &         0.651  $\pm{0.005}$ &         1.352  $\pm{0.002}$ &         0.473  $\pm{0.007}$ &          0.697  $\pm{0.022}$ &         -0.779  $\pm{0.013}$ &          0.670  $\pm{0.028}$ &         -0.450  $\pm{0.014}$ \\
% MPANP (ours)           & \textBF{1.374} $\pm{0.000}$ & \textBF{0.698} $\pm{0.007}$ & \textBF{1.373} $\pm{0.001}$ & \textBF{0.501} $\pm{0.005}$ &         1.167 $\pm{0.047}$ & \textBF{-0.628} $\pm{0.027}$ & \textBF{ 0.773} $\pm{0.039}$ & \textBF{-0.446} $\pm{0.057}$ \\
        \bottomrule
    \end{tabular}}
\end{table}

==> table/_old_tables/table_gp_robust.tex <==
\begin{table}[t]
    \caption{Results of Robustness among kernels experiments. Context and target log likelihood values on data sampled from Gaussian Processes with various kernels. Here we first trained models on RBF dataset and evaluate performances on various settings.  Performances are measured over 4 seeds.\\}
    \label{tab:table_gp_robust}
    \centering
    \scriptsize
    \renewcommand{\arraystretch}{0.85}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lrrrrrrrrrrrr}
        \toprule
        \multirow{3}{*}{Model} & \multicolumn{2}{r}{RBF}                                   & \multicolumn{2}{r}{Matern}                                & \multicolumn{2}{r}{Periodic}                                & \multicolumn{2}{r}{$t$-noise}                               \\
                                 \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                          \cmidrule(lr){6-7}                                            \cmidrule(lr){8-9}
                               & context                     & target                      & context                     & target                      & context                      & target                       & context                      & target                       \\
        \midrule
CNP                    &         0.964  $\pm{0.006}$ &         0.288  $\pm{0.006}$ &         0.826  $\pm{0.007}$ &         0.076  $\pm{0.007}$ &         -0.504  $\pm{0.045}$ &         -2.686  $\pm{0.087}$ &          0.151  $\pm{0.101}$ &         -2.382  $\pm{0.011}$ \\
NP                     &         0.951  $\pm{0.007}$ &         0.299  $\pm{0.007}$ &         0.804  $\pm{0.008}$ &         0.076  $\pm{0.015}$ &         -0.421  $\pm{0.011}$ &         -2.430  $\pm{0.110}$ &         -0.336  $\pm{1.016}$ &         -2.177  $\pm{0.157}$ \\
BNP                    &         1.020  $\pm{0.006}$ &         0.372  $\pm{0.006}$ &         0.890  $\pm{0.006}$ &         0.192  $\pm{0.007}$ & \textBF{-0.281} $\pm{0.004}$ & \textBF{-1.265} $\pm{0.009}$ &  \textBF{0.455} $\pm{0.001}$ & \textBF{-1.329} $\pm{0.092}$ \\
NeuBNP                 &         0.929  $\pm{0.011}$ &         0.275  $\pm{0.007}$ &         0.806  $\pm{0.012}$ &         0.109  $\pm{0.006}$ &         -0.378  $\pm{0.028}$ &         -1.730  $\pm{0.037}$ &          0.314  $\pm{0.077}$ &         -1.406  $\pm{0.184}$ \\
MPNP (ours)            & \textBF{1.086} $\pm{0.005}$ & \textBF{0.457} $\pm{0.002}$ & \textBF{0.967} $\pm{0.007}$ & \textBF{0.261} $\pm{0.005}$ &         -0.314  $\pm{0.026}$ &         -1.448  $\pm{0.025}$ &          0.104  $\pm{0.240}$ &         -1.638  $\pm{0.241}$ \\
\cmidrule(lr){1-1}       \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                          \cmidrule(lr){6-7}                                            \cmidrule(lr){8-9}
CANP                   &         1.372  $\pm{0.000}$ &         0.611  $\pm{0.008}$ &         1.367  $\pm{0.001}$ &         0.427  $\pm{0.006}$ &          0.312  $\pm{0.111}$ &         -6.607  $\pm{0.268}$ &          0.980  $\pm{0.045}$ &         -2.889  $\pm{0.094}$ \\
ANP                    &         1.372  $\pm{0.003}$ &         0.616  $\pm{0.026}$ &         1.367  $\pm{0.004}$ &         0.427  $\pm{0.028}$ &          0.445  $\pm{0.137}$ &         -6.521  $\pm{0.437}$ &          1.009  $\pm{0.025}$ &         -2.868  $\pm{0.120}$ \\
BANP                   & \textBF{1.374} $\pm{0.001}$ &         0.663  $\pm{0.002}$ &         1.370  $\pm{0.001}$ &         0.476  $\pm{0.006}$ &          0.731  $\pm{0.046}$ &         -3.165  $\pm{0.322}$ &          1.092  $\pm{0.011}$ &         -2.269  $\pm{0.170}$ \\
NeuBANP                &         1.357  $\pm{0.002}$ &         0.651  $\pm{0.005}$ &         1.347  $\pm{0.002}$ &         0.467  $\pm{0.007}$ & \textBF{ 0.970} $\pm{0.020}$ & \textBF{-2.300} $\pm{0.228}$ &  \textBF{1.169} $\pm{0.008}$ &         -2.090  $\pm{0.120}$ \\
MPANP (ours)           & \textBF{1.374} $\pm{0.000}$ & \textBF{0.699} $\pm{0.007}$ & \textBF{1.370} $\pm{0.001}$ & \textBF{0.500} $\pm{0.004}$ &          0.616  $\pm{0.042}$ &         -3.551  $\pm{0.092}$ &          1.016  $\pm{0.080}$ & \textBF{-2.071} $\pm{0.097}$ \\
        \bottomrule
    \end{tabular}}
\end{table}

==> table/_old_tables/table_image.tex <==
\begin{table}[t]
    \caption{Context and target log likelihood values of image completion tasks on MNIST, CIFAR10, and CelebA datasets. Performances are measured over 3 seeds.\\}
    \label{tab:table_image}
    \centering
    \scriptsize
    \renewcommand{\arraystretch}{0.9}
    \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{lrrrrrrrrrr}
        \toprule
        \multirow{3}{*}{Model} & \multicolumn{2}{r}{MNIST}                                 & \multicolumn{2}{r}{SVHN}                               & \multicolumn{2}{r}{CelebA}                                \\
                                 \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                          \cmidrule(lr){6-7}
                               & context                     & target                      & context                     & target                      & context                     & target                      \\
        \midrule
CNP                    &         1.119  $\pm{0.003}$ &         0.814  $\pm{0.003}$ &         3.512  $\pm{0.010}$ &         3.175  $\pm{0.006}$ &         3.701  $\pm{0.002}$ &         3.370  $\pm{0.001}$ \\
NP                     &         1.084  $\pm{0.003}$ &         0.801  $\pm{0.002}$ &         3.393  $\pm{0.012}$ &         3.104  $\pm{0.004}$ &         3.681  $\pm{0.006}$ &         3.366  $\pm{0.005}$ \\
BNP                    & \textBF{1.143} $\pm{0.001}$ &         0.845  $\pm{0.001}$ &         3.575  $\pm{0.004}$ &         3.244  $\pm{0.002}$ &         3.730  $\pm{0.004}$ &         3.413  $\pm{0.003}$ \\
NeuBNP                 &         1.104  $\pm{0.001}$ &         0.871  $\pm{0.001}$ &         3.506  $\pm{0.008}$ &         3.244  $\pm{0.005}$ &         3.682  $\pm{0.002}$ &         3.415  $\pm{0.001}$ \\
MPNP (ours)            &         1.134  $\pm{0.001}$ & \textBF{0.886} $\pm{0.001}$ & \textBF{3.628} $\pm{0.003}$ & \textBF{3.305} $\pm{0.003}$ & \textBF{3.758} $\pm{0.005}$ & \textBF{3.460} $\pm{0.003}$ \\
\cmidrule(lr){1-1}       \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                          \cmidrule(lr){6-7}
CANP                   & \textBF{1.383} $\pm{0.000}$ &         0.860  $\pm{0.001}$ & \textBF{4.148} $\pm{0.000}$ &         3.575  $\pm{0.025}$ & \textBF{4.150} $\pm{0.000}$ &         3.656  $\pm{0.001}$ \\
ANP                    &         1.381  $\pm{0.002}$ &         0.830  $\pm{0.025}$ &         4.144  $\pm{0.002}$ &         3.566  $\pm{0.016}$ &         4.149  $\pm{0.000}$ &         3.648  $\pm{0.006}$ \\
BANP                   & \textBF{1.383} $\pm{0.000}$ &         0.859  $\pm{0.014}$ & \textBF{4.148} $\pm{0.000}$ &         3.567  $\pm{0.037}$ & \textBF{4.150} $\pm{0.000}$ &         3.651  $\pm{0.007}$ \\
NeuBANP                &         1.371  $\pm{0.001}$ &         0.893  $\pm{0.007}$ &         4.137  $\pm{0.002}$ &         3.580  $\pm{0.007}$ &         4.139  $\pm{0.000}$ &         3.646  $\pm{0.001}$ \\
MPANP (ours)           & \textBF{1.383} $\pm{0.000}$ & \textBF{0.950} $\pm{0.002}$ & \textBF{4.148} $\pm{0.000}$ & \textBF{3.645} $\pm{0.008}$ & \textBF{4.150} $\pm{0.000}$ & \textBF{3.694} $\pm{0.004}$ \\
% CNP                    &         1.114  $\pm{0.004}$ &         0.765  $\pm{0.005}$ &         3.538  $\pm{0.010}$ &         3.124  $\pm{0.007}$ &         3.702  $\pm{0.002}$ &         3.274  $\pm{0.002}$ \\
% NP                     &         1.080  $\pm{0.003}$ &         0.754  $\pm{0.002}$ &         3.430  $\pm{0.010}$ &         3.077  $\pm{0.001}$ &         3.681  $\pm{0.006}$ &         3.275  $\pm{0.007}$ \\
% BNP                    & \textBF{1.139} $\pm{0.000}$ &         0.796  $\pm{0.002}$ &         3.596  $\pm{0.003}$ &         3.196  $\pm{0.002}$ &         3.730  $\pm{0.004}$ &         3.326  $\pm{0.002}$ \\
% NeuBNP                 &         1.100  $\pm{0.001}$ &         0.828  $\pm{0.001}$ &         3.534  $\pm{0.009}$ &         3.215  $\pm{0.005}$ &         3.683  $\pm{0.002}$ &         3.340  $\pm{0.002}$ \\
% MPNP (ours)            &         1.129  $\pm{0.001}$ & \textBF{0.847} $\pm{0.002}$ & \textBF{3.642} $\pm{0.003}$ & \textBF{3.248} $\pm{0.004}$ & \textBF{3.759} $\pm{0.004}$ & \textBF{3.381} $\pm{0.003}$ \\
% \cmidrule(lr){1-1}       \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                          \cmidrule(lr){6-7}
% CANP                   & \textBF{1.383} $\pm{0.000}$ &         0.801  $\pm{0.004}$ & \textBF{4.148} $\pm{0.000}$ &         3.451  $\pm{0.027}$ & \textBF{4.150} $\pm{0.000}$ &         3.556  $\pm{0.001}$ \\
% ANP                    &         1.381  $\pm{0.002}$ &         0.777  $\pm{0.021}$ &         4.143  $\pm{0.002}$ &         3.443  $\pm{0.018}$ & \textBF{4.149} $\pm{0.000}$ &         3.549  $\pm{0.007}$ \\
% BANP                   & \textBF{1.383} $\pm{0.000}$ &         0.801  $\pm{0.011}$ &         4.147  $\pm{0.000}$ &         3.448  $\pm{0.049}$ & \textBF{4.149} $\pm{0.000}$ &         3.561  $\pm{0.006}$ \\
% NeuBANP                &         1.371  $\pm{0.001}$ &         0.838  $\pm{0.007}$ &         4.136  $\pm{0.002}$ &         3.470  $\pm{0.008}$ &         4.139  $\pm{0.000}$ &         3.550  $\pm{0.001}$ \\
% MPANP (ours)           & \textBF{1.383} $\pm{0.000}$ & \textBF{0.892} $\pm{0.003}$ & \textBF{4.148} $\pm{0.000}$ & \textBF{3.537} $\pm{0.009}$ & \textBF{4.149} $\pm{0.000}$ & \textBF{3.606} $\pm{0.006}$ \\
        \bottomrule
    \end{tabular}}
\end{table}


==> table/_old_tables/table_lotka.tex <==
\begin{table}[t]
    \caption{Context and target log likelihood values on Lotka Volterra simulated data and real data. Performances are measured over 4 seeds.\\}
    \label{tab:table_lotka}
    \centering
    \scriptsize
    \renewcommand{\arraystretch}{0.9}
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{lrrrr}
        \toprule
        \multirow{3}{*}{Model} & \multicolumn{2}{r}{Simulation}                            & \multicolumn{2}{r}{Real}                                    \\
                                 \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                       
                               & context                     & target                      & context                     & target                        \\
        \midrule
        CNP                    &         0.161  $\pm{0.038}$ &        -0.192  $\pm{0.032}$ &         -2.759  $\pm{0.027}$ &         -3.278  $\pm{0.041}$ \\
        NP                     &         0.185  $\pm{0.036}$ &        -0.152  $\pm{0.037}$ &         -2.707  $\pm{0.027}$ &         -3.200  $\pm{0.042}$ \\
        BNP                    &         0.402  $\pm{0.009}$ &         0.038  $\pm{0.018}$ &         -2.723  $\pm{0.032}$ &         -3.168  $\pm{0.041}$ \\
        NeuBNP                 &         0.114  $\pm{0.059}$ &        -0.267  $\pm{0.053}$ &         -2.794  $\pm{0.073}$ &         -3.128  $\pm{0.045}$ \\
        MPNP (ours)            & \textBF{0.403} $\pm{0.047}$ & \textBF{0.116} $\pm{0.035}$ & \textBF{-2.648} $\pm{0.041}$ & \textBF{-3.106} $\pm{0.021}$ \\
        \cmidrule(lr){1-1}       \cmidrule(lr){2-3}                                          \cmidrule(lr){4-5}                                       
        CANP                   &         2.498  $\pm{0.018}$ &         1.541  $\pm{0.010}$ &          1.836  $\pm{0.169}$ &         -6.873  $\pm{0.612}$ \\
        ANP                    &         2.528  $\pm{0.026}$ &         1.643  $\pm{0.011}$ & \textBF{ 2.058} $\pm{0.080}$ &         -5.454  $\pm{0.408}$ \\
        BANP                   & \textBF{2.605} $\pm{0.021}$ &         1.685  $\pm{0.032}$ &          2.054  $\pm{0.126}$ & \textBF{-3.388} $\pm{0.446}$ \\
        NeuBANP                &         2.421  $\pm{0.024}$ &         1.358  $\pm{0.026}$ &          1.878  $\pm{0.050}$ &         -3.739  $\pm{0.240}$ \\
        MPANP (ours)           &         2.554  $\pm{0.025}$ & \textBF{1.769} $\pm{0.013}$ &          1.946  $\pm{0.136}$ &         -4.942  $\pm{0.387}$ \\
        \bottomrule
    \end{tabular}}
\end{table}
